Collaborative Generative AI: Integrating GPT-k for Efficient Editing in Text-to-Image Generation

The field of text-to-image (T2I) generation has garnered significant attention both within the research community and among everyday users. Despite the advancements of T2I models, a common issue encountered by users is the need for repetitive editing of input prompts in order to receive a satisfactory image, which is time-consuming and labor-intensive. Given the demonstrated text generation power of large-scale language models, such as GPT-k, we investigate the potential of utilizing such models to improve the prompt editing process for T2I generation. We conduct a series of experiments to compare the common edits made by humans and GPT-k, evaluate the performance of GPT-k in prompting T2I, and examine factors that may influence this process. We found that GPT-k models focus more on inserting modifiers while humans tend to replace words and phrases, which includes changes to the subject matter. Experimental results show that GPT-k are more effective in adjusting modifiers rather than predicting spontaneous changes in the primary subject matters. Adopting the edit suggested by GPT-k models may reduce the percentage of remaining edits by 20-30%.

==> tables/image_similarity_all.tex <==
\begin{table*}[t]
\begin{adjustbox}{width=\linewidth,center}
\begin{tabular}{l|rrrrr|rrrrr|rrrrr}\toprule
\multirow{2}{*}{\textbf{Model}} &\multicolumn{5}{c|}{\textbf{SSIM}} &\multicolumn{5}{c|}{\textbf{PSNR}}  &\multicolumn{5}{c}{\textbf{CLIP cosine similarity}} \\\cmidrule{2-16}
&$\vi_{1}$-$\vi_{n}$ &$\vi_{n-1}$-$\vi_{n}$ &$\vi'$-$\vi_{n}$ &$\vi'$-$\vi_{MS}$ &RNE &$\vi_{1}$-$\vi_{n}$ &$\vi_{n-1}$-$\vi_{n}$ &$\vi'$-$\vi_{n}$ &$\vi'$-$\vi_{MS}$ &RNE &$\vi_{1}$-$\vi_{n}$ &$\vi_{n-1}$-$\vi_{n}$ &$\vi'$-$\vi_{n}$ &$\vi'$-$\vi_{MS}$ &RNE  \\\midrule
\texttt{gpt2-base} &\multirow{8}{*}{18.93} &\multirow{8}{*}{20.39} &17.60 &22.99 &52.32 &\multirow{8}{*}{9.16} &\multirow{8}{*}{9.37} &9.35 &10.44 &52.92 &\multirow{8}{*}{71.72} &\multirow{8}{*}{74.82} &69.58 &80.16 &75.28 \\
\texttt{gpt2-medium} & & &17.54 &22.96 &52.60 & & &9.36 &10.45 &53.30 & & &69.63 &80.39 &78.28 \\
\texttt{gpt2-large} & & &17.52 &22.94 &52.80 & & &9.36 &10.45 &52.57 & & &69.70 &80.50 &78.88 \\
\texttt{gpt2-xl} & & &17.51 &22.86 &52.98 & & &9.35 &10.44 &53.29 & & &69.57 &80.37 &75.25 \\
\texttt{gpt3-ada} & & &17.11 &22.28 &53.71 & & &9.33 &10.37 &52.67 & & &66.95 &76.37 &69.43 \\
\texttt{gpt3-babbage} & & &16.97 &22.12 &52.85 & & &9.26 &10.30 &52.40 & & &68.79 &78.81 &72.33 \\
\texttt{gpt3-curie} & & &17.41 &22.80 &53.51 & & &9.29 &10.36 &52.25 & & &68.45 &78.28 &71.41 \\
\texttt{gpt3.5-davinci} & & &16.91 &22.00 &51.92 & & &9.22 &10.27 &52.32 & & &68.79 &78.09 &69.22 \\
\bottomrule
\end{tabular}
\end{adjustbox}

\caption{
The automatic evaluation metrics scores to evaluate image similarity. Here, $\vi_1$, $\vi_{n-1}$, $\vi_n$ denotes the first, last-but-one, and last image in the trace of edits; $\vi'$ is the image generated from the modified prompt, and $\vi_{MS}$ is the image that is most similar to $\vi'$ with regard to current similarity metric.
}
\label{tab:image_similarity_auto}

\end{table*}

==> tables/trace_examples/eg1.tex <==
\begin{table}[h]
\begin{adjustbox}{width=\linewidth,center}
\begin{tabular}{lc}
\textbf{User Input Prompt} & \textbf{Generated Image} \\
\toprule
\makecell[lt]{
\texttt{circular ornated ceiling highly detailed}
}
& \includegraphics[align=t,width=3cm]{figures/eg_traces/trace1/0.png}\\
\midrule

\makecell[lt]{
\texttt{ornated circular ceiling, with paintings}\\
\texttt{of angels, highly detailed}
}
& \includegraphics[align=t,width=3cm]{figures/eg_traces/trace1/1.png}\\
\midrule

\makecell[lt]{
\texttt{photo of an ornated circular ceiling, full of}\\
\texttt{paintings of angels, centered symmetrical}\\
\texttt{highly detailed}
}
& \includegraphics[align=t,width=3cm]{figures/eg_traces/trace1/2.png}\\
\midrule

\makecell[lt]{
\texttt{photo of an ornated circular ceiling, full of}\\
\texttt{paintings of angels, centered symmetrical}\\
\texttt{highly detailed}
}
& \includegraphics[align=t,width=3cm]{figures/eg_traces/trace1/3.png}\\
\midrule

\makecell[lt]{
\texttt{ornate marble and gold wall, full of}\\
\texttt{paintings of angels, highly detailed}
}
& \includegraphics[align=t,width=3cm]{figures/eg_traces/trace1/4.png}\\
\midrule

\makecell[lt]{
\texttt{ornate wall, full of paintings of angels,}\\
\texttt{highly detailed}
}
& \includegraphics[align=t,width=3cm]{figures/eg_traces/trace1/5.png}\\
\midrule

\makecell[lt]{
\texttt{ornate wall, full of paintings of angels,}\\
\texttt{unreal engine texture highly detailed}
}
& \includegraphics[align=t,width=3cm]{figures/eg_traces/trace1/6.png}\\


% \makecell[lt]{\texttt{

% }}
% & \includegraphics[align=t,width=3cm]{figures/eg_traces/trace1/6.png}\\

\end{tabular}
\end{adjustbox}
    \caption{Caption for the whole figure}
    \label{fig:fig1}
\end{table}




